Adaptive Incremental Mixture Markov chain Monte Carlo

We propose Adaptive Incremental Mixture Markov chain Monte Carlo (AIMM), a novel approach to sample from challenging probability distributions defined on a general state-space. While adaptive MCMC methods usually update a parametric proposal kernel with a global rule, AIMM locally adapts a semiparametric kernel. AIMM is based on an independent Metropolis-Hastings proposal distribution which takes the form of a finite mixture of Gaussian distributions. Central to this approach is the idea that the proposal distribution adapts to the target by locally adding a mixture component when the discrepancy between the proposal mixture and the target is deemed to be too large. As a result, the number of components in the mixture proposal is not fixed in advance. Theoretically, we prove that there exists a process that can be made arbitrarily close to AIMM and that converges to the correct target distribution. We also illustrate that it performs well in practice in a variety of challenging situations, including high-dimensional and multimodal target distributions.

==> New folder (2)/mfmr18_appendices.tex <==
\begin{appendices}


\section{Proof of Proposition \ref{prop1}}
\label{app1}

\setcounter{condition}{0}
%\setcounter{proposition}{0}
\setcounter{corollary}{0}


In this appendix, we use the following notations
\begin{itemize}
\item $\tQ_n$ is the incremental part of the proposal $Q_n$ at iteration $n$, \ie $\tQ_n\propto\sum_{k=1}^{n-1}\beta_k\phi_k$
\item at iteration $n$, only $M_n\leq n-1$ components among $\phi_1,\ldots,\phi_{n-1}$ have a non-zero weight
\item $\event_n$ is the event that the proposal increments at iteration $n$ of AIMM, \ie $\beta_n>0$ almost surely
\item $\event$ is the event that the proposal increments infinitely often \ie $\event=\cap_n\cup_{k>n}\event_n$
\end{itemize}


The proof of Proposition \ref{prop1} is achieved by first showing that the KL divergence between $\tQ_n$ and $\tQ_{n+1}$ goes to zero. This allows to prove that, in the total variation norm, $\{Q_n\}_n$ adapts less and less and finally that the convergence to zero of the difference between two consecutive transition kernels $K_n-K_{n+1}$ occurs uniformly, provided that some implementation details are satisfied. We first state the following lemma and a corollary that will be needed to establish the diminishing adaptation for the AIMM process.

\begin{lemma}
\label{lemma:1}
The sum of the weights $\bbeta_n$ is not bounded in $\proba_\event$-probability, \ie
$\bbeta_n\overset{\proba_\event}{\to}\infty$.
\end{lemma}

\begin{proof}
Let $M>0$, and note that
\begin{multline}
\label{eq:app:lem1_1}
\proba_\event\{\bbeta_{n+1}<M\}=\proba_\event\{\bbeta_{n+1}<M\,\cap\, \bbeta_{n}<M\}+\proba_\event\{\bbeta_{n+1}<M\,\cap\, \bbeta_{n}\geq M\}\\
=\proba_\event\{\bbeta_{n+1}<M\,|\, \bbeta_{n}<M\}\proba_\event\{\bbeta_n<M\}\leq \proba_\event\{\bbeta_n<M\}
\end{multline}
since $\proba_\event\{\bbeta_{n+1}<M\,\cap\, \bbeta_{n}\geq M\}\leq \proba_\event\{\bbeta_{n+1}<M\,|\, \bbeta_{n}\geq M\}\leq \proba_\event\{\bbeta_{n+1}<\bbeta_n\,|\,\bbeta_n\geq M\}=0$. Note that the inequality in \eqref{eq:app:lem1_1} is strict on $\event_n$. Indeed,
\begin{equation}
\label{eq:app:lem1_2}
\proba_\event\{\beta_{n+1}\geq M-\bbeta_n\,|\, \bbeta_{n}<M,\event_n\}>0\Rightarrow
\proba_\event\{\bbeta_{n+1}< M\,|\, \bbeta_{n}<M,\event_n\}<1\,,
\end{equation}
while
\begin{equation}
\label{eq:app:lem1_3}
%\proba\{\beta_{n+1}\geq M-\bbeta_n\,|\, \bbeta_{n}<M,\overline{\event_n}\}=0\Rightarrow
\proba_\event\{\bbeta_{n+1}< M\,|\, \bbeta_{n}<M,\overline{\event_n}\}=1\,.
\end{equation}

Combining \eqref{eq:app:lem1_1}, \eqref{eq:app:lem1_2} and \eqref{eq:app:lem1_3} shows that $\{\proba_\event\{\bbeta_n<M\}\}_n$ is a decreasing sequence. In particular, it is strictly decreasing an infinite number of times and therefore $\proba_\event\{\bbeta_{n}<M\}\to 0$ which yields $\bbeta_n\overset{\proba_\event}{\to}\infty$.
\end{proof}

\begin{corollary}
\label{coro:1}
On $\event$, the incremental component weight \ie $\beta_n/\bbeta_n$ goes to zero in probability.
\end{corollary}
\begin{proof}
Let $\eps>0$ and note that since $\pi$ is absolutely continuous we have $\sup_{x\in\Xset}\pi(x)=:\bar{\pi}<\infty$ and
\begin{equation}
\label{eq:app:lem1_0}
\proba_\event\left\{\frac{\pi(\tX_n)^\gamma}{\bbeta_n}>\eps\right\}\leq  \proba_\event \left\{\frac{\bar{\pi}^\gamma}{\bbeta_n}>\eps\right\}\,.
\end{equation}
Using Lemma \ref{lemma:1}, the RHS of \eqref{eq:app:lem1_0}  goes to zero as $n\to\infty$ which concludes the proof.

\end{proof}


\subsection{Diminishing adaptation in the KL metric and total variation norm}
\begin{proposition}
\label{prop:2}
Assume that almost surely
\begin{enumerate}[\textbf{A}1.]
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\end{enumerate}
Consider the sequence $\{\tD_n\}_{n>0}$, defined as the KL divergence between the incremental components of two consecutive proposals, i.e.~$\tD_n=\KL\{\tQ_n,\tQ_{n+1}\}$. Then $\tD_n$ converges to zero in probability, \ie $\tD_n=o_\proba(1)$.
\end{proposition}

\begin{proof}
\label{proof2}
For all $\eps>0$, we have
\begin{equation}
\label{eq:app:1}
\proba\{\tD_n>\eps\}=\proba\{\tD_n>\eps\cap\bar{\event}\}+\proba\{\tD_n>\eps\cap\event\}\,.
\end{equation}
We will show that both terms in the RHS of Eq. \eqref{eq:app:1} converge to 0.

For the first term, note that $\bar{\event}$ is the event that the mixture will eventually stop incrementing.  Therefore for all $\omega\in\bar{\event}$, there exists $\nu\in\nset$ such that for all $n>n_0$, $\tQ_n=\tQ_{n+1}$. Hence, for any $n>n_0$, $\omega\not\in\{\tD_n>\eps\}$. This implies that $\{\tD_n>\eps\}$ and $\bar{\event}$ are eventually mutually exclusive events, leading to the first term in the RHS of Eq. \eqref{eq:app:1} converging to 0.

We now show that the second term in the RHS of Eq. \eqref{eq:app:1} goes to zero. The case where $\proba(\event)=0$ is trivial. Indeed, $\proba(\event)=0\Rightarrow \proba\{\tD_n>\eps\cap\event\}=0$ and the proof is completed. In the following, we consider the case where $0<\proba(\event)\leq 1$ and show that $\proba\{\tD_n>\eps\cap\event\}$ converge to 0 as well. First, note that we have
\begin{equation}
\label{eq:app:1_2}
\proba\{\tD_n>\eps\cap\event\}\leq \proba\{\tD_n>\eps\,|\,\event\}\,.
\end{equation}
Defining $\bbeta_n=\sum_{k\leq n}\beta_k$, we now show that the RHS of Eq. \eqref{eq:app:1_2} goes to zero in probability.
\begin{multline*}
\tD_n=\int\rmd\tQ_n \log \frac{\tQ_n}{\tQ_{n+1}}\leq \int\rmd\tQ_n \log \frac{\tQ_n}{\tQ_{n+1}}=
\int\rmd\tQ_n \log \frac{\sum_{k=1}^{n-1}\beta_k\phi_k}{\sum_{k=1}^{n}\beta_k\phi_k}\times \frac{\bar{\beta}_{n}}{\bar{\beta}_{n-1}}\\
\leq \int\rmd\tQ_n \left|\log \frac{\sum_{k=1}^{n-1}\beta_k\phi_k}{\sum_{k=1}^{n}\beta_k\phi_k}\right|+\int\rmd\tQ_n\left| \log\frac{\bar{\beta}_{n}}{\bar{\beta}_{n-1}}\right|=
\int\rmd\tQ_n \log \frac{\sum_{k=1}^{n}\beta_k\phi_k}{\sum_{k=1}^{n-1}\beta_k\phi_k}+ \log\frac{\bar{\beta}_{n}}{\bar{\beta}_{n-1}}\,,
\end{multline*}
where the last equality holds since for all $x\in\Xset$, $\sum_{k=1}^{n-1}\beta_k\phi_k(x)\leq \sum_{k=1}^{n}\beta_k\phi_k(x)$. Since we assume that $\pi$ is absolutely continuous, there exists a finite constant $\overline{\pi}>0$ such that for all $x\in\Xset$, the pdf of $\pi$ satisfies $\pi(x)<\overline{\pi}$, which implies that $\beta_{n}<\overline{\pi}^\gamma$. Using the log inequality, this yields:
$$
\tD_n\leq \overline{\pi}^\gamma\left\{\int\rmd\tQ_n \frac{\phi_{n}}{\sum_{k=1}^{n-1}\beta_k\phi_k}+ \frac{1}{\bar{\beta}_{n-1}}\right\}=
\frac{\overline{\pi}^\gamma}{\bbeta_{n-1}} \left\{1+\int\rmd\phi_n\right\}\,,%\\=
%\frac{1}{\sum_{k=1}^{M_n} b_k} \left\{1+\int\rmd\phi_{M_n+1}W_n\frac{Q_n}{\tQ_n}\right\}\,,
$$
 We now write that by inclusion of events,
$$
\proba_\event\{\tD_n>\eps\}\leq
\proba_\event\left\{\frac{2\overline{\pi}^\gamma}{\bbeta_{n-1}}>\eps\right\}=\proba_\event\left\{\bbeta_{n+1}\leq \frac{2\overline{\pi}^\gamma}{\eps}\right\}\,.
$$
The proof is completed by applying Lemma \ref{lemma:1}.
\end{proof}

\begin{proposition}
\label{prop:3}
Assume that almost surely
\begin{enumerate}[\textbf{A}1.]
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\end{enumerate}
The sequence of random variables $\{D_n:=\KL\{Q_n,Q_{n+1}\}\}_{n>0}$ goes to zero in probability.
\end{proposition}

\begin{proof}
By straightforward algebra, we have:
\begin{multline*}
\label{eq:Dn}
D_n=\int\rmd Q_n\log\frac{Q_n}{Q_{n+1}}=\omega_n\int\rmd Q_0\log \frac{Q_n}{Q_{n+1}}+(1-\omega_n)\int\rmd \tQ_n\log \frac{Q_n}{Q_{n+1}}\\
\leq
\omega_n\int\rmd Q_0\log \frac{Q_0+(1-\omega_n)\tQ_n}{\omega_{n+1}Q_0}+
(1-\omega_n)\int\rmd \tQ_n\log \frac{\omega_nQ_0+(1-\omega_n)\tQ_n}{(1-\omega_{n+1})\tQ_{n+1}}\\
=
\omega_n\int\rmd Q_0\log \frac{ Q_0}{\omega_{n+1}Q_0}\left\{1+\frac{(1-\omega_n)\tQ_n}{Q_0}\right\}+
(1-\omega_n)\int\rmd \tQ_n\log \frac{(1-\omega_n)\tQ_n}{(1-\omega_{n+1})\tQ_{n+1}}\left\{1+\frac{\omega_nQ_0}{(1-\omega_n)\tQ_n}\right\}\\
\leq
\omega_n\log \frac{1}{\omega_{n+1}}+\omega_n\int\rmd Q_0\log \left\{1+\frac{(1-\omega_n)\tQ_n}{Q_0}\right\}
+(1-\omega_n)\tD_n+(1-\omega_n)\int\rmd \tQ_n\log \left\{1+\frac{\omega_nQ_0}{(1-\omega_n)\tQ_n}\right\}\\
\leq
\omega_n\log \frac{1}{\omega_{n+1}}+(1-\omega_n)\tD_n
+\omega_n\int\rmd Q_0\frac{(1-\omega_n)\tQ_n}{Q_0}
+(1-\omega_n)\int\rmd \tQ_n\frac{\omega_nQ_0}{(1-\omega_n)\tQ_n}\\
=
\omega_n\log \frac{1}{\omega_{n+1}}+(1-\omega_n)\tD_n
+\omega_n{(1-\omega_n)}
+(1-\omega_n)\frac{\omega_n}{(1-\omega_n)}
\leq
\tD_n+v_n\,,
\end{multline*}
where we have used the log inequality $\log(1+x)< x$ for all $x>0$ and defined $v_n:=-\omega_n\log {\omega_{n+1}}+2\omega_n$.
The proof is completed by noting that
\begin{equation}
\label{eq:Dn4}
\proba\{D_n>\eps\}\leq \proba\{\tD_n+v_n>\eps\}
\end{equation}
and applying Proposition \ref{prop:2} to get that $\tD_n=o_{\proba}(1)$ which, combined with the fact that $v_n=o(1)$, shows that the RHS of Eq. \eqref{eq:Dn4} converges to zero.
\end{proof}

\begin{corollary}
Assume that almost surely
\begin{enumerate}[\textbf{A}1.]
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\end{enumerate}
Then the difference between two consecutive proposals converges in total variation to zero in probability, \ie $\left\|Q_n-Q_{n+1}\right\|=o_\proba(1)$.
\end{corollary}

\begin{proof}
This result follows from combining Proposition \ref{prop:2} together with Pinsker inequality,
\begin{equation}
\label{eq:pinsker}
\|Q_n-Q_{n+1}\|\leq \sqrt{\frac{1}{2}\KL\{Q_n,Q_{n+1}\}}\,.
\end{equation}
Indeed, for all $\eps>0$, we have using Eq. \eqref{eq:pinsker} that
$$
\proba\{\|Q_{n}-Q_{n+1}\|^2>\eps\}\leq \proba\{\KL\{Q_n,Q_{n+1}\}>2\eps\}\,,
$$
which shows that $\|Q_n-Q_{n+1}\|^2=o_\proba(1)$. The proof is completed by using the continuous mapping theorem since $x\mapsto\sqrt{x}$ is continuous on $[0,1]$ and therefore preserves the limit.
\end{proof}


\subsection{Diminishing adaptation in the sup norm}
We want to prove that
$$
\sup_{x\in\Xset}\|K_{n+1}(x,\cdot)-K_{n}(x,\cdot)\| ,
$$
converges to zero in probability, which corresponds to the diminishing assumption of \cite{roberts2007}. We first establish the following result.



\begin{proposition}
\label{prop:unif}
Assume that almost surely
\begin{enumerate}[\textbf{A}1]
\setcounter{enumi}{0}
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\end{enumerate}
Then the difference between two consecutive proposal probability density functions converge uniformly to zero in probability \ie $\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|=o_{\proba}(1)$.
\end{proposition}
\begin{proof}
Let $\eps>0$, we will show that $\lim_n\proba\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\}= 0$. Using similar arguments to those in the proof of Proposition \ref{prop:2}, we have that
\begin{multline*}
\proba\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\right\}=\proba\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\,\cap\, \event\right\}\\
+\underbrace{\proba\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\,\cap\, \bar{\event}\right\}}_{\searrow 0 }\,,
\end{multline*}
and
\begin{equation*}
\proba\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\,\cap\, \event\right\}\leq
\proba_\event\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\right\}\,.%\\
%=\proba\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps\,\cap\,\event_n \,|\, \event\}\leq
%\proba\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps \,|\, \event,\event_n\}\,.
\end{equation*}
Now by straightforward algebra we have that
\begin{multline}
\label{eq:prop:unif1}
|Q_{n+1}(x)-Q_n(x)|=\left|(\omega_{n+1}-\omega_n)Q_0(x)+\frac{1-\omega_{n+1}}{\bbeta_{n+1}}\sum_{k=1}^{{M_n}+1}\beta_k\phi_k(x)-
\frac{1-\omega_{n}}{\bbeta_{n}}\sum_{k=1}^{M_n}\beta_k\phi_k(x)\right|\\
\leq \frac{\kappa}{(1+\kappa n)(1+\kappa(n+1))}Q_0(x)+\sum_{k=1}^{M_n} \beta_k\phi_k(x)\left|\frac{1-\omega_{n+1}}{\bbeta_{n+1}}-\frac{1-\omega_{n}}{\bbeta_{n}}\right|+\frac{\beta_{M_n+1}}{\bbeta_{n+1}}\phi_{M_n+1}(x)\\
\leq \frac{\kappa}{(1+\kappa n)^2}{Q_0}(x)+(1-\omega_{n})\left|1-\frac{(1-\omega_{n+1})\bbeta_n}{(1-\omega_n)\bbeta_{n+1}}\right|\tQ_n(x)+\frac{\beta_{M_n+1}}{\bbeta_{n+1}}{\phi_{M_n+1}}(x)\\
\leq\frac{\kappa}{(1+\kappa n)^2}\overline{Q_0}+\left|1-\frac{1-\omega_{n+1}}{1-\omega_n}\left(1-\frac{\beta_{M_n+1}}{\bbeta_{n+1}}\right)\right|\overline{\tQ_n}+\frac{\beta_{M_n+1}}{\bbeta_{n+1}}\overline{\phi_{M_n+1}}=:R_n\,,
\end{multline}
where for any real-valued function $f:\Xset\to\rset$, we have defined $\overline{f}:=\sup_{x\in\Xset}{f}(x)$. Since $\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|\leq R_n$, we have that
$$
\proba_\event\left\{\sup_{x\in\Xset}|Q_{n+1}(x)-Q_n(x)|>\eps \right\}\leq
\proba_\event\left\{R_n>\eps \right\}\,.
$$
The proof is concluded by noting that $R_n$ is the sum of three random variables, each of which converges to zero in $\proba_\event$-probability:
\begin{itemize}
\item ${\kappa\overline{Q_0}}/{(1+\kappa n)^2}=o(1)$,
\item the middle term in \eqref{eq:prop:unif1} is upper bounded by
$$
\left|1-\frac{1-\omega_{n+1}}{1-\omega_n}\left(1-\frac{\beta_{M_n+1}}{\bbeta_{n+1}}\right)\right|\leq \left|1-\frac{1-\omega_{n+1}}{1-\omega_n}\right|+
\frac{\beta_{M_n+1}}{\bbeta_{n+1}}\frac{1-\omega_{n+1}}{1-\omega_n}
$$
and noting that ${1-\omega_{n+1}}\slash {1-\omega_n}\to 1$, the first terms converges to zero surely and, using Corollary \ref{coro:1}, the second one converges to zeros in $\proba_\event$-probability,
\item the last term converges to zero in $\proba_\event$-probability, again using Corollary \ref{coro:1}.
\end{itemize}
\end{proof}

\begin{proposition}
\label{prop:cauchy}
Assume that
\begin{enumerate}[\textbf{A}1.]
\setcounter{enumi}{0}
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\item the incremental mixture (unnormalized) weights are defined as:
\begin{equation}
\label{eq:new_weights}
\beta_n=\frac{\eta+\pi(\tX_n)^\gamma}{(1+\eta)^n}\1_{\event_n}
\qquad\text{and}\qquad\omega_n=\frac{1}{1+\sum_{k=1}^n\beta_k}\,,
\end{equation}
where $\eta>0$ is a constant, typically $\eta\ll 1$.
\end{enumerate}
Then, $\{Q_n\}_n$ converges uniformly in probability to a distribution $Q$, \ie $\sup_{x\in\Xset}|Q_n(x)-Q(x)|=o_\proba(1)$
\end{proposition}
\begin{proof}
Uniform convergence being equivalent to uniformly Cauchy, we show that $\{Q_n\}_n$ is uniformly Cauchy, in probability, \ie
\begin{equation}
\label{unifCauchy}
\sup_{x\in\Xset}\sup_{\ell\in\nset}|Q_{n+\ell}(x)-Q_n(x)|=o_\proba(1)\,.
\end{equation}
Using the same reasoning that in the proof of Proposition \ref{prop:2}, it is sufficient to prove that the convergence occurs in $\proba_\event$-probability only. Similarly to Proposition \ref{prop:unif}, we write
$$
|Q_{n+\ell}-Q_n|\leq |\omega_{n+\ell}-\omega_n|\overline{Q_0}+\left|\frac{1-\omega_{n+\ell}}{\bbeta_{n+\ell}}-\frac{1-\omega_n}{\bbeta_n}\right|
\sum_{k=1}^n\beta_k\overline{\phi_k}+\frac{1}{\bbeta_{n+\ell}}\sum_{k=n+1}^{n+\ell}\beta_k\overline{\phi_k}\,,
$$
where we have used the same notations than in the proof of Proposition \ref{prop:unif}.

First, we note that
\begin{equation}
\label{eq:step1}
|\omega_{n+\ell}-\omega_n|=\frac{\omega_0(\bbeta_{n+\ell}-\bbeta_n)}{(\omega_0+\bbeta_n)(\omega_0+\bbeta_{n+\ell})}\leq \frac{\bbeta_{n+\ell}-\bbeta_n}{\omega_0}
\end{equation}
and since
\begin{equation}
\label{eq:bbeta}
\bbeta_{n+\ell}-\bbeta_n=\sum_{k=n+1}^{n+\ell}\frac{\eta+\pi(\tX_k)^\gamma}{(1+\eta)^k}\leq \frac{\eta+\overline{\pi}^\gamma}{(1+\eta)^n}\sum_{k=1}^\ell\frac{1}{(1+\eta)^k}=
\frac{\eta+\overline{\pi}^\gamma}{(1+\eta)^n}\frac{1-\{1/(1+\eta)\}^\ell}{\eta}\,,
\end{equation}
clearly $|\omega_{n+\ell}-\omega_n|\leq{(\eta+\overline{\pi}^\gamma)}(1+\eta)^{-n}\slash{\eta\omega_0}$. Second, we have
\begin{equation*}
\left|\frac{1-\omega_{n+\ell}}{\bbeta_{n+\ell}}-\frac{1-\omega_n}{\bbeta_n}\right|=\left|\frac{1}{\omega_0+\bbeta_{n+\ell}}-\frac{1}{\omega_0+\bbeta_n}\right|\leq \frac{\bbeta_{n+\ell}-\bbeta_n}{\omega_0^2}\leq\frac{{(\eta+\overline{\pi}^\gamma)}}{\eta \omega_0^2(1+\eta)^n}
\end{equation*}
Moreover, by assumption \textbf{A}2, we have that $\overline{\phi_k}\leq 1/(2\pi)^{d/2}\sqrt{\delta}$, so
$$
\sum_{k=1}^n\beta_k\overline{\phi_k}\leq \frac{1}{(2\pi)^{d/2}\sqrt{\delta}}\bbeta_n\,.
$$
Since
$$
\bbeta_n\leq {\eta+\overline{\pi}^\gamma}\sum_{k=1}^n\frac{1}{(1+\eta)^k}=\frac{\eta+\overline{\pi}^\gamma}{\eta}\{1-(1/(1+\eta))^n\}<
\frac{\eta+\overline{\pi}^\gamma}{\eta}\,,
$$
we have that
\begin{equation}
\label{eq:step2}
\left|\frac{1-\omega_{n+\ell}}{\bbeta_{n+\ell}}-\frac{1-\omega_n}{\bbeta_n}\right|\sum_{k=1}^n\beta_k\overline{\phi_k}\leq
\frac{{(\eta+\overline{\pi}^\gamma)}^2}{\eta^2 \omega_0^2(2\pi)^{d/2}\sqrt{\delta}}\frac{1}{(1+\eta)^n}\,.
\end{equation}
Finally, using Eq. \eqref{eq:bbeta}, we have
\begin{equation}
\label{eq:step3}
\frac{1}{\bbeta_{n+\ell}}\sum_{k=n+1}^{n+\ell}\beta_k\overline{\phi_k}\leq \frac{\bbeta_{n+\ell}-\bbeta_n}{\omega_0}\leq
\frac{\eta+\overline{\pi}^\gamma}{\eta\omega_0(1+\eta)^n}\,.
\end{equation}
Combining Eqs. \eqref{eq:step1}, \eqref{eq:bbeta}, \eqref{eq:step2} and \eqref{eq:step3}, we have that
\begin{equation}
\label{eq:step4}
|Q_{n+\ell}(x)-Q_n(x)|\leq Z_n:=\frac{1}{(1+\eta)^n}\frac{\eta+\overline{\pi}^\gamma}{\eta\omega_0}\left\{1+\overline{Q_0}+\frac{\eta+\overline{\pi}^\gamma}{\eta\omega_0}\right\}\,,
\end{equation}
so that for all $\eps>0$,
$$
\proba_\event\left\{\sup_{x,\ell}|Q_{n+\ell}(x)-Q_n(x)|>\eps\right\}\leq \proba_\event\{Z_n>\eps\}
$$
which converges to zero as $\{Z_n\}_{n}$ is a deterministic sequence that converges to zero. The proof is completed.
\end{proof}


\begin{proposition}
\label{prop:cauchy_reciprocate}
Assume that
\begin{enumerate}[\textbf{A}1.]
\setcounter{enumi}{0}
\item the covariance matrix of any component of the mixture satisfies $\det\Sigma_k>\delta>0$
\item the incremental mixture (unnormalized) weights are defined as:
\begin{equation}
\label{eq:new_weights}
\beta_n=\frac{\eta+\pi(\tX_n)^\gamma}{(1+\eta)^n}\1_{\event_n}
\qquad\text{and}\qquad\omega_n=\frac{\omega_0}{\omega_0+\sum_{k=1}^n\beta_k}\vee \lambda\,,
\end{equation}
where $\eta>0$ and $\lambda\in(0,1)$ are some constants, typically $(\eta,\lambda)\ll 1$.
\item the initial kernel $Q_0$ is subexponential or satisfies $Q_0(x)\propto \exp\{\psi(x)\}$ where $\psi=o(x^2)$ $(x\to\infty)$, \ie $Q_0$ has heavier tail than a Gaussian, \eg multivariate Laplace or t-distribution.
\end{enumerate}

Then, the function $\{H_n:=1/Q_n\}_n$ converges uniformly in probability to a function $H$, \ie $\sup_{x\in\Xset}|H_n(x)-H(x)|=o_\proba(1)$
\end{proposition}

\begin{proof}
As in the proof of Proposition \ref{prop:cauchy}, we show that $\{H_n\}_n$ is uniformly Cauchy convergent in probability. Under Assumption \textbf{A}2, we have that for all $x\in\Xset$ and $\ell\in\nset$, for $n$ sufficiently large, $\omega_n=\lambda$ and
$$
Q_n=\lambda Q_0+(1-\lambda)\frac{\sum_{k=1}^{n}\beta_k\phi_k}{\bbeta_n}\,.
$$
\begin{multline*}
|H_{n+\ell}-H_n|=\frac{|Q_{n+\ell}-Q_n|}{Q_{n+\ell}Q_n}\\
=\frac{(1-\lambda)\left|\sum_{k=1}^{n+\ell}\beta_k\phi_k/\bbeta_{n+\ell}-\sum_{k=1}^{n}\beta_k\phi_k/\bbeta_{n}\right|}{\left(\lambda Q_0+(1-\lambda){\sum_{k=1}^{n}\beta_k\phi_k}\slash{\bbeta_n}\right)\left(\lambda Q_0+(1-\lambda){\sum_{k=1}^{n+\ell}\beta_k\phi_k}\slash{\bbeta_{n+\ell}}\right)}\\
\leq
\frac{(1-\lambda)}{\lambda^2Q_0^2}\left|\sum_{k=1}^{n}\beta_k\phi_k\left(\frac{1}{\bbeta_{n+\ell}}-\frac{1}{\bbeta_n}\right)+
\frac{1}{\bbeta_{n+\ell}}\sum_{k=n+1}^{n+\ell}\beta_k\phi_k\right|\\
\leq \frac{(1-\lambda)}{\lambda^2}\left\{\left|\frac{1}{\bbeta_{n+\ell}}-\frac{1}{\bbeta_n}\right|\sum_{k=1}^{n}\beta_k\frac{\phi_k}{Q_0^2}
+\frac{1}{\bbeta_{n+\ell}}\sum_{k=n+1}^{n+\ell}\beta_k\frac{\phi_k}{Q_0^2}\right\}\\
\leq \frac{(1-\lambda)}{\lambda^2\bbeta_n^2}\left\{{\sum_{k=n+1}^{n+\ell}\beta_k}\sum_{k=1}^{n}\beta_k\frac{\phi_k}{Q_0^2}
+\bbeta_n\sum_{k=n+1}^{n+\ell}\beta_k\frac{\phi_k}{Q_0^2}\right\}\,.
\end{multline*}
Now by assumption \textbf{A}3. the function ${\phi_k}/{Q_0^2}$ is bounded for all $x\in\Xset$ and there exists $M<\infty$ such that for any Gaussian pdf $\phi$, $\phi/Q_0^2<M$. This yields:
$$
\sup_{x\in\Xset}|H_{n+\ell}(x)-H_n(x)|\leq
2\frac{(1-\lambda)M}{\lambda^2\bbeta_n}{\sum_{k=n+1}^{n+\ell}\beta_k}\leq Y_n:=2\frac{(1-\lambda)M}{\lambda^2\bbeta_n}\frac{\eta+\overline{\pi}^\gamma}{\eta(1+\eta)^n}\,.
$$
Upon $\event$, for $n$ sufficiently large $\bbeta_n>0$ almost surely and $Y_n\to 0$. The proof is completed by noting that
$$
\proba_\event\left\{\sup_{x,\ell}|H_{n+\ell}(x)-H_n(x)|>\eps\right\}\leq \proba_\event\{Y_n>\eps\}\to 0\,.
$$
\end{proof}

\begin{corollary}
\label{coro:2}
Assume that assumptions \textbf{A}1, \textbf{A}2 and \textbf{A}3 of Proposition \ref{prop:cauchy_reciprocate} hold, then
$$
\sup_{x\in\Xset}\left|1-\frac{Q_n(x)}{Q(x)}\right|=o_\proba(1)\,.
$$
\end{corollary}
\begin{proof}
We have
$$
\sup_{x\in\Xset}\left|1-\frac{Q_n(x)}{Q(x)}\right|=\sup_{x\in\Xset}Q_n(x)\left|\frac{1}{Q_n(x)}-\frac{1}{Q(x)}\right|\leq \sup_{x\in\Xset}Q_n(x)\sup_{x\in\Xset}\left|\frac{1}{Q_n(x)}-\frac{1}{Q(x)}\right|\,,
$$
and the proof is completed by noting that, for a sufficiently large $n$, we have
$$
Q_n\leq \lambda \overline{Q_0}+(1-\lambda)\frac{1}{(2\pi)^{d/2}\sqrt{\delta}}
$$
and applying Proposition \ref{prop:cauchy_reciprocate}.
\end{proof}

We can now prove Proposition \ref{prop1}
\setcounter{proposition}{0}
\begin{proposition}
\label{prop:diminish_cauchy}
Assume that \textbf{A}1--\textbf{A}3 of Proposition \ref{prop:cauchy_reciprocate} hold and that in addition, we have:
\begin{enumerate}[\textbf{A}1.]
\setcounter{enumi}{3}
\item the event $\event_n$ upon which the mixture increments is defined with $\uW>0$
\end{enumerate}
Then, AIMM satisfies diminishing adaptation, \ie
$$
\sup_{x\in\Xset}\|K_{n+1}(x,\cdot)-K_n(x,\cdot)\|=o_{\proba}(1)\,.
$$
\end{proposition}

\begin{proof}
From Proposition \ref{prop:cauchy}, we know that there exists a probability density function $Q$ such that $\{Q_n\}_n$ converges uniformly to $Q$. Denoting by $K$ the MH transition kernel with proposal $Q$, we have that
$$
\|K_{n+1}(x,\cdot)-K_n(x,\cdot)\|\leq \|K_{n}(x,\cdot)-K(x,\cdot)\|+\|K_{n+1}(x,\cdot)-K(x,\cdot)\|\,.
$$
To establish diminishing adaptation, it is thus sufficient to prove that $\sup_{x\in\Xset}\|K_{n}(x,\cdot)-K(x,\cdot)\|=o_{\proba_\event}(1)$. In particular, we can write
\begin{multline}
\label{eq:dimish3}
\|K_{n}(x,\cdot)-K(x,\cdot)\|=\int\left|(Q(y)-Q_n(y))\alpha(x,y)-Q_n(y)(\alpha_n(x,y)-\alpha(x,y))\right|\rmd y+\\
\left|\int\alpha(x,y)(Q(y)-Q_n(y))\rmd y-\int Q_n(\rmd y)(\alpha_n(x,y)-\alpha(x,y))\right|\\
\leq 2\sup_{x\in\Xset}\left|Q(x)-Q_n(x)\right|+2\int Q_n(\rmd y)\left|\alpha_n(x,y)-\alpha(x,y)\right|\,.
\end{multline}
Now note that for all $(x,y)\in\Xset^2$,
$$
\left|\alpha_n(x,y)-\alpha(x,y)\right|\leq \left|\frac{\pi(y) Q_n(x)}{\pi(x)Q_n(y)}-\frac{\pi(y) Q(x)}{\pi(x)Q(y)}\right|
$$
we have
\begin{multline}
\label{eq:dimish2}
\int Q_n(\rmd y)\left|\alpha_n(x,y)-\alpha(x,y)\right|\leq \int \frac{\pi(y)}{\pi(x)}\left|Q_n(x)-\frac{Q(x)Q_n(y)}{Q(y)}\right|\rmd y\\
\leq
\int \frac{\pi(y)}{\pi(x)}\left|Q_n(x)-Q(x)+Q(x)\left(\frac{Q_n(y)}{Q(y)}-1\right)\right|\rmd y\\
\leq
\int \frac{\pi(y)}{\pi(x)}\left|Q_n(x)-Q(x)\right|\rmd y+\int \frac{W(y)}{W(x)}\left|{Q_n(y)}-Q(y)\right|\rmd y\\
\leq \int \frac{\pi(y)}{W(x)}\left|1-\frac{Q_n(x)}{Q(x)}\right|\rmd y+\int \frac{W(y)}{W(x)}\left|{Q_n(y)}-Q(y)\right|\rmd y
\leq \frac{2}{\underline{W}}\sup_{x\in\Xset}\left|1-\frac{Q_n(x)}{Q(x)}\right|\,.%\\
%\leq \left(\frac{1}{\inf_{x\in\Xset} \pi(x)}+\frac{\Wst}{\underline{W}}\right)\sup_{x\in\Xset}\left|{Q_n(x)}-Q(x)\right|\,.
\end{multline}
Indeed, the proposal limit $Q$ must satisfy $\underline{W}<W:=\pi/Q<\Wst$. Combining Eqs. \eqref{eq:dimish3} and \eqref{eq:dimish2} yields
$$
\sup_{x\in\Xset}\|K_{n}(x,\cdot)-K(x,\cdot)\|\leq 2\left(\sup_{x\in\Xset}\left|{Q_n(x)}-Q(x)\right|+\frac{1}{\underline{W}}\sup_{x\in\Xset}\left|1-\frac{Q_n(x)}{Q(x)}\right|\right)\,,
$$
and applying Proposition \ref{prop:cauchy} and Corollary \ref{coro:2} completes the proof.
\end{proof}

\section{Proof of Proposition \ref{prop2}}
\label{app2}
We show that the AIMM version presented in Section \ref{sec:conv:aimm2} satisfies diminishing adaptation and containment and is thus ergodic \cite[Theorem 2]{roberts2007}.

\subsection{Diminishing Adaptation}
First we note that diminishing adaptation is implied by Assumption \textbf{B}3. Indeed, using the same approach that in Appendix \ref{app1} and introducing the quantity $\overline{\Delta}_n:=\sup_{x\in\Xset}\|\overline{P}_{n+1}(x,\,\cdot\,)-\overline{P}_{n}(x,\,\cdot\,)\|$, we have for all $\eps>0$
\begin{equation}
\label{eq:app2:1}
\proba\{\overline{\Delta}_n>\eps\}=\proba\{\overline{\Delta}_n>\eps\,|\,\event\}\proba\{\event\}+\proba\{\overline{\Delta}_n>\eps\,|\,\event^c\}
\proba\{\event^c\}\,,
\end{equation}
where for readability we have denoted by ${\event}^c$ the complementary event of ${\event}$ ($\event=\cap_n\cup_{k>n}\event_k$). Now on $\event^c$, there exists a $n_0<\infty$ such that for all $n>n_0$ the mixture does not increment anymore. In such a case, $\proba\{\overline{\Delta}_n>\eps\,|\,\event^c\}=0$ as soon as $n>n_0$ since for all $n>n_0$, $\proba\{M_n=M_{n_0}\}=1$. This implies that $\proba\{\overline{P}_{n+1}(x,\,\cdot\,)=\overline{P}_{n}(x,\,\cdot\,)\}=1$ which is straightforward if $\omega_n$ is a function of $n$ through $M_n$. Now by definition of $\overline{\event}=\cap_n\cup_{k>n}\overline{\event}_k$ ($\overline{\event}_n=\event_n\cap \{M_n<M\}$), upon $\event$, there exists an $n_1<\infty$ such that $M_{n_1}=M$ and for all $n>n_1$, $\proba\{M_n=M\}=1$. Similarly to the reasoning with $\event^c$, we conclude that for all $n>n_1$, $\proba\{\overline{\Delta}_n>\eps\,|\,\event\}=0$. Diminishing adaptation follows from Eq. \ref{eq:app2:1} by writing that for all $\eps>0$ and $n>\max(n_0,n_1)$, $\proba\{\overline{\Delta}_n>\eps\}=0$.


\subsection{Containment}
We now show that under the Assumptions of Proposition \ref{prop2}, the AIMM process satisfies the containment condition \ie $C_n(\eps)$ defined at Eq. \eqref{eq:cont} is bounded in probability. We use Theorem 1 from \cite{rosenthal2017ergodicity}, which extends the seminal development made in \cite{craiu2015stability} and in particular Theorem 21 therein. In \cite{rosenthal2017ergodicity}, adaptive MCMC are analysed in a parametric adaptation framework, \ie under the assumption that there exists a set $\Ycal\subset \rset^p$ such that any adaptive proposal belongs to a family of distributions parameterized by $\Ycal$. Theorem 1 \citep{rosenthal2017ergodicity} identifies six assumptions, that we now enumerate for completeness, that are sufficient to guarantee the containment condition. We define for all $r>0$, $\comp_r:=\{x\in\Xset,\,\min_{y\in\comp}\|x-y\|\leq r\}$.
\begin{enumerate}[\textbf{RY}-1]
\item $\Ycal$ is compact.
\item The process evolves through a $\pi$-Harris ergodic transition kernel that does not allow moves larger than some fixed distance $D>0$.
\item The process only adapts within a compact set $\comp$.
\item $Q_0$ is bounded above by $Q_0(\rmd y)\leq \zeta \nu_\ast(\rmd y)$ where $\nu_\ast$ is a probability measure concentrated on $\comp_{2D}\backslash \comp_D$.
\item There exists two positive constants $(\varepsilon,\delta)$ such that the fixed kernel $P$, \ie the M-H kernel with proposal $Q_0$, is bounded below by $P(x,\rmd y)\geq \varepsilon \text{Leb}(\rmd y)$ whenever $(x,y)\in J$ with $\|x-y\|\leq \delta$ and $J\supset \comp_{2D}\backslash \comp_D$.
\item The function $(x,y,\gamma)\mapsto Q_\gamma(x,y)$ is combocontinuous, \ie it is a finite combination of continuous functions (which generalizes the concept of piecewise continuous functions where some pieces are not necessarily intervals).
\end{enumerate}
We now show that all those assumptions are satisfied by the AIMM process described at Section \ref{sec:conv:aimm2}.

In the context of Proposition \ref{prop2}, we define $\Ycal$ as the following union of sets
\begin{equation}
\label{eq:app2:2}
\Ycal:=\cup_{\ell=0}^M\left\{\mathsf{A}^\ell,\mathsf{B}^\ell,\mathsf{C}^\ell\right\}\,,
\end{equation}
such that $\mathsf{A}:=\{\beta\in\rset,\;0\leq \beta\leq \overline{\pi}^\gamma\}$, $\mathsf{B}:=\{\mu\in\rset^d,\;-L\leq \mu_i\leq L\}$ and
$\mathsf{C}:=\{\Sigma\in\mathcal{M}_d(\rset),\;-L\leq \Sigma_{i,j}\leq L\}$. Indeed for all $n\in\nset$, there exists $\gamma=\{\beta_1,\ldots,\beta_\ell,\mu_1,\ldots,\mu_\ell,\Sigma_1,\ldots,\Sigma_\ell\}$ with $\ell\leq M$ such that  $\oQ_n^\comp\equiv\oQ_{\gamma}^\comp:=\overline{\omega}_n^\comp Q_0+(1-\overline{\omega}_n^\comp)\sum_{l=1}^\ell\beta_l\Phi(\,\cdot\,|\,\mu_l,\Sigma_l)\slash \sum_{l=1:\ell}\beta_l$ and $\gamma\in\Ycal$. Clearly, $\Ycal$ is a finite union of compact sets and is thus compact and \textbf{RY}-1 holds. By construction, the second part of \textbf{RY}-2 and \textbf{RY}-3 hold. Moreover, it can be noted that for any $D>0$, the Metropolis algorithm that consists in proposing $\tX_{n+1}\sim \overline{Q}_n^\comp$ and accepting with probability $\1_{\|\tX_{n+1}-X_n\|\leq D}\overline{\alpha}^\comp(X_n,\tX_{n+1})$, with $\overline{\alpha}^\comp$ is defined as $\alpha$ \eqref{eq:alpha} up to replacing $Q_n$ by $\overline{Q}_n^\comp$, is still $\pi$-invariant. This follows from noting that this algorithm would generate a $\pi$-reversible Markov chain. Since it is also $\phi$-irreducible and aperiodic, $\oP_\gamma^\comp$ is Harris ergodic for $\pi$, for any $\gamma\in\Ycal$. This checks \textbf{RY}-2. \textbf{RY}-4 is straightforward by taking $Q_0$ as any distribution dominated by the Lebesgue measure, \eg multivariate Gaussian, multivariate T-student, etc. Assumption \textbf{RY}-5 follows from $Q_0$ and $\pi$ being absolutely continuous distributions on $(\Xset,\Xalg)$. Finally, we note that for a fixed $\gamma\in\Ycal$, $(x,y)\mapsto \oQ^\comp_\gamma(x,y)$ is piecewise continuous. In fact this function is continuous on the two complementary sets $\comp$ and $\overline{\kappa}$. Moreover, we note that for a fixed $y\in\Xset$, $(\gamma,x)\mapsto \oQ_\gamma^\comp(x,y)=\sum_{l=1}^M\1_{\ell(\gamma)=l}\oQ_{\gamma}^\comp(x,y)$, where $\ell(\gamma)$ is the number of components in the mixture $\oQ_\gamma^\comp$. Since for all $\ell\in\{0,\ldots,M\}$, $x\in\Xset$, the mapping $(x,\gamma)\mapsto \oQ_{\gamma}^\comp(x,y)$ is piecewise continuous, $(\gamma,x)\mapsto \oQ_\gamma^\comp(x,y)$ is combocontinuous and \textbf{RY}-6 holds. The proof is completed.

\section{Simulation details}
\label{app5}
\subsection{Competing algorithms}
\label{app:alg}
\begin{itemize}
\item Adaptive Metropolis--Hastings (AMH) \citep{haario2001adaptive}: a benchmark adaptive MCMC algorithm with non-independence proposal kernel
\begin{equation*}
Q_n(x_n,\cdot)=\left\{
\begin{array}{lc}
\Psi_d(\,\cdot\,;\,x_n,\Sigma_0) & \text{if}\; n\leq N_0\\
p\Psi_d(\,\cdot\,;\,x_n,\Sigma_0) +(1-p)\Psi_d(\,\cdot\,;\,x_n,\Sigma_n) & \text{otherwise}
\end{array}
\right.
\end{equation*}
where $\Psi_d(\,\cdot\,;\,m,S)$ is the $d$-dimensional Gaussian distribution with mean $m$, covariance matrix $S$, $\Sigma_0$ is an initial covariance matrix and $N_0$
the number of preliminary iterations where no adaptation is made. We consider the version of AMH proposed in \cite{roberts2009examples}, in which there is a strictly positive
probability ($p=.05$) of proposing through the initial Gaussian random walk. The covariance matrix of the adaptive part of the proposal is written $\Sigma_n=s_d\Gamma_n$,
where $\Gamma_n$ is defined as the empirical covariance matrix from all the previous states of the $X_1,\ldots,X_n$, and $s_d=2.4^2/d$ is a scaling factor.
The parameters $N_0$ and $\Sigma_0$ were set to be equal to the corresponding AIMM parameters.

\item Adaptive Gaussian Mixture Metropolis--Hastings (AGM) \citep{luengo2013fully}: an adaptive MCMC with an independence proposal kernel defined as a mixture of
Gaussian distributions
    \begin{equation}
    Q_n=\sum_{\ell=1}^{M}\omega_{\ell,n}\Psi_d(\,\cdot\,;\,\mu_{\ell,n},\Lambda_{\ell,n})\,.
    \end{equation}
    In AGM, the number of components $M$ is fixed. The proposal distribution $Q_n$ is parameterised by the vector
    $\Omega_n=\{\omega_{\ell,n},\mu_{\ell,n},\Lambda_{\ell,n}\}_{\ell=1}^M$. Given the new state $X_{n+1}$ of the chain, the next parameter $\Omega_{n+1}$ will
    follow from a deterministic update ; see \cite[section 4]{luengo2013fully} for more details. In the implementation, we set the number of components $M$ identical to the corresponding AIMM parameter $\Mmax$.

\item For the sake of comparing with non--adaptive methods, we also include the Independence Sampler (IM) (see \eg \cite{liu1996metropolized}) and the random
walk Metropolis--Hastings (RWMH) (see \eg \cite{roberts2001optimal}) using the Matlab build--in function \textit{mhsample} with default settings.
\end{itemize}


\subsection{Performance indicators}
\label{app:perf}
The quality of a sampler is based on its ability to explore the state space fully and quickly without getting trapped in specific states (mixing). The KL divergence between $\targ$ and the chain distribution (if available) and the \textit{Effective Sample Size} are indicators that allow us to assess those two properties. Related statistics such as the chain \textit{Jumping distance} and the \textit{Acceptance rate} of the sampler are also reported. We also provide the chain \textit{Efficiency}, which penalizes the Effective Sample Size by the computational burden generated by the sampler.

\begin{itemize}
\item For a stochastic process $\{X_k,\,k\leq n\}$, we recall that when sampling from $\targ$ is feasible, the KL divergence between the target and the chain distribution can be approximated by
    \begin{equation}
    \KL=\frac{1}{L}\sum_{\ell=1}^L\log\left\{\frac{\targ(Z_\ell)}{\Law(Z_\ell\,|\,X_{1:n})}\right\}\,, \quad Z_\ell\sim \targ\,,
    \end{equation}
    where $\Law(\,\cdot\,|\,X_{1:n})$ is the kernel density estimation of the stochastic process (obtained using the routine \texttt{ksdensity} provided in Matlab in the default setting). We stress that using approximated values for $\KL$ are not an issue here as we are first and foremost interested in comparing different samplers, with lower KL being the better.

\item The jumping distance measures how fast the sampler explores the state space, see \cite{pasarica2010adaptively}. For a stochastic process $\{X_k,\,k\leq n\}$
it is estimated by:
\begin{equation}
\JMP=\frac{1}{n-1}\sum_{k=1}^{n-1}\|X_{k+1}-X_k\|^2 ,
\end{equation}
and the larger the squared distance the better.

\item The mixing rate of a of a one dimensional chain $(d=1)$ is classically evaluated with the Effective Sample Size (ESS), which is approximated by
\begin{equation}
\label{eq:ess}
\ESS=1\bigg\slash \left\{1+2\sum_{t=1}^T\hat{\rho}_{t}\right\}\, ,
\end{equation}
where $\hat{\rho}_{t}$ denotes the empirical lag $t$ covariance estimated using the sample path of $X_{1:n}$, $T=\min(1000,t_0)$ and $t_0$ is the smaller lag such that $\hat{\rho}_{t_0+\ell}<.01$, for all $\ell>0$. $\text{ESS}\in(0,1)$ (ESS=1 corresponds to \iid samples) and the higher $\ESS$, the better the algorithm. When $d>1$, $\ESS$ is set as the minimum ESS among the $d$ marginal ESS's.

\item The tradeoff between the computational efficiency and the precision is estimated by $\EFF$
\begin{equation}
\EFF=\ESS\bigg\slash\tau\,,
\end{equation}
where $n$ is the total number of iterations performed by the sampler and $\tau$ the CPU time (in second) required to achieve the $N$ transitions
\citep{tran2014adaptive}.
\end{itemize}

\subsection{AGM targeting $\pi_2$}
\label{app:agm}
Although similar to AIMM, AGM adapts a Gaussian mixture proposal to the target, the distribution of the resulting chain remains far from $\pi_2$ after $200,000$
iterations. Figure \ref{fig:banana_agm} gives a hint to understand why AGM is not efficient in sampling from $\pi_2$. By construction, AGM adapts locally a component of the proposal, provided that some samples are available in its vicinity. As a result, components initially located where the probability mass is non-negligible will adapt well to the target but the others will see their weight shrinking to zero (in dimension two, out of one hundred initial kernels having the same weight, the ten kernels with highest weight hold $0.99$ of the total mixture weight after $200,000$ iterations). This gives those kernels with initial poor location a high inertia, which prevents them moving away from low density regions to reach regions that are yet to be supported by the proposal. AIMM's opportunistic increment process explores the state space more efficiently.

\begin{figure}
\centering
\includegraphics[scale=.42]{initial_prop_dim2-eps-converted-to.pdf}
\includegraphics[scale=.42]{initial_prop_dim10-eps-converted-to.pdf}

\includegraphics[scale=.42]{final_prop_dim2-eps-converted-to.pdf}
\includegraphics[scale=.42]{final_prop_dim10-eps-converted-to.pdf}

\includegraphics[scale=.152]{samples_dim2.png}
\includegraphics[scale=.152]{samples_dim10.png}
\caption{(example \ref{example_pi2}) $\pi_2$ target, $d\in\{2,10\}$ - AGM sampling from $\pi_2$ in dimensions $d=2$ (left column) and $d=10$ (right column, projection onto the first two dimensions). First and second rows: initial mixtures with centers drawn uniformly and adapted mixtures after $n=200,000$ iterations. The grey levels on the ellipses stand for the weights of the components (from white to black for larger weights) and the region inside the ellipses contains $75\%$ of each Gaussian mass. Third row: samples $\{X_{1,2},X_{2,n}\,,n\leq 200,000\}$ from AGM. \label{fig:banana_agm}}
\end{figure}

\end{appendices} 
